Searches for Large-Scale Anisotropy in the Arrival Directions of Cosmic Rays Detected above Energy of $10^{19}$ eV at the Pierre Auger Observatory and the Telescope Array

Spherical harmonic moments are well-suited for capturing anisotropy at any scale in the flux of cosmic rays. An unambiguous measurement of the full set of spherical harmonic coefficients requires full-sky coverage. This can be achieved by combining data from observatories located in both the northern and southern hemispheres. To this end, a joint analysis using data recorded at the Telescope Array and the Pierre Auger Observatory above $10^{19}$ eV is presented in this work. The resulting multipolar expansion of the flux of cosmic rays allows us to perform a series of anisotropy searches, and in particular to report on the angular power spectrum of cosmic rays above $10^{19}$ eV. No significant deviation from isotropic expectations is found throughout the analyses performed. Upper limits on the amplitudes of the dipole and quadrupole moments are derived as a function of the direction in the sky, varying between 7% and 13% for the dipole and between 7% and 10% for a symmetric quadrupole.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 3255 2014-01-14 10:20:10Z veberic $

USEPDFLATEX := 1
USEBIBTEX := 0

TARGET := augerta
DEPENDENCIES := $(wildcard figs/*) author_list-auger.tex author_list-ta.tex

##########################################################

LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)

COLORIZE := awk 'BEGIN{red="\033[31;1m";yel="\033[34m";byel="\033[34;1m";end="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print red""$$0""end;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print yel""$$0""end;next}{print}END{if(w||e)print "\n"red"Warning/error summary:\n"byel""w""end;if(e){print red""e""end;exit 1}}'

define basic_latex_rule
  for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
endef

ifeq ($(USEBIBTEX), 1)
define latex_rule
  $(LATEX) $< ; bibtex $*
  $(call basic_latex_rule)
endef
else
define latex_rule
  $(call basic_latex_rule)
endef
endif

.PHONY: all clean

all: author_list-auger.tex author_list-ta.tex $(TARGET).pdf

# dependencies
$(TARGET).pdf: $(DEPENDENCIES)

clean:
	- for e in .tex~ .ps .pdf .dvi .log .aux .toc .nav .out .snm .bbl .blg .spl .lof Notes.bib .maf .fff .lot .ttt ; do rm -f $(TARGET)$$e ; done
	- rm -f author_list-auger.tex author_list-ta.tex

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf %.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.ps
	ps2pdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<

author_list-auger.tex: auger/*
	(cd auger ; sh ../aastex-authors.shawk) >$@

author_list-ta.tex: ta/*
	(cd ta ; sh ../aastex-authors.shawk) >$@

